RoT: Enhancing Table Reasoning with Iterative Row-Wise Traversals

The table reasoning task, crucial for efficient data acquisition, aims to answer questions based on the given table. Recently, reasoning large language models (RLLMs) with Long Chain-of-Thought (Long CoT) significantly enhance reasoning capabilities, leading to brilliant performance on table reasoning. However, Long CoT suffers from high cost for training and exhibits low reliability due to table content hallucinations. Therefore, we propose Row-of-Thought (RoT), which performs iteratively row-wise table traversal, allowing for reasoning extension and reflection-based refinement at each traversal. Scaling reasoning length by row-wise traversal and leveraging reflection capabilities of LLMs, RoT is training-free. The sequential traversal encourages greater attention to the table, thus reducing hallucinations. Experiments show that RoT, using non-reasoning models, outperforms RLLMs by an average of 4.3%, and achieves state-of-the-art results on WikiTableQuestions and TableBench with comparable models, proving its effectiveness. Also, RoT outperforms Long CoT with fewer reasoning tokens, indicating higher efficiency.

==> old_version/1.introduction_0510.tex <==
% 引出表格推理任务
% 表格推理是一项很重要的任务，其输入包括表格和问题，输出为根据表格对问题的回答
Table reasoning is an important task where the input consists of a question and the table, and the output is the answer based on the table \cite{jin2022table-survey,zhang2025table-survey}. 
% 其中表格由多个并列的行组成，而每行由多个cell组成，包含着大量密集的信息
Tables typically comprise multiple rows, with each row containing several information-dense cells \cite{ruan2024table-data-survey}.
% 由于自动化的表格推理可以帮助人们从表格中抽取出有效信息，提升数据获取效率，收到很多研究者关注
Automated table reasoning attracts considerable research interest due to its potential to extract valuable information from tables, thus accelerating data acquisition \cite{badaro-etal-2023-transformers-table-survey,lu2025table-survey}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{fig/intro.pdf}
    % \vspace{-1.5em}
    \caption{
    % 我们的方法training-free且能更好地激发模型的表格推理能力
    \ours is training-free and can enhance the table reasoning ability better, compared with Long CoT with RLLMs.
    }
    \label{fig:intro}
\end{figure}

% 推理模型及其缺点，引出我们的方法
% 近些年，推理模型凭借引入Long CoT显著提升了模型的推理能力，比如在数学、程序生成等任务上
Recent advancements in reasoning large language models (RLLMs) have significantly enhanced reasoning capabilities utilizing Long Chain-of-Thought (Long CoT), particularly in domains such as mathematics and coding \cite{openai2024openai-o1-card,guo2025deepseek-r1,li202512survey-reasoning}. 
% Long CoT推理指的是模型可以自主选择或切换推理路径，进行足够深的逐步推理，相比较短CoT浅显、直接的推理
Long CoT refers to autonomously selecting or switching reasoning paths and performing sufficiently deep step-by-step reasoning, in contrast to the shallow and direct reasoning in Short CoT \cite{chen2025reasoning-survey,xu2025redstar,yeo2025demystifying-long-cot}.  
% 然而，目前的推理模型具备以下缺点
However, current RLLMs exhibit the following limitations:
% Low Reliability: 模型频繁地切换推理路径容易导致模型遗漏或对表格中的信息产生幻觉，从而出错
(\emph{i})~\textbf{Low Reliability}: Frequent transitions between reasoning paths can lead to omissions or hallucinations regarding tabular information, resulting in errors \cite{shi-etal-2024-trusting-Evidence-Hallucinate, Liu2025hallucination-long,zeng2025revisiting-test-truly,yin2025distillation-bottleneck}. 
(\emph{ii})~\textbf{High Cost}: Enhancing table reasoning capabilities of non-reasoning LLMs necessitates high-quality Long CoT data, leading to substantial training expenses \cite{qian2025fino1,jiang2024slow1,qin2024o1-replication}.
% High Cost: 想要进一步增强表格的推理能力需要高质量的Long CoT数据，所以训练成本大
% 然而，获得Long CoT的能力需要通过SFT或强化学习训练，which需要高质量的数据，并且resource-intensive
% However, acquiring Long CoT capabilities necessitates high-quality Long CoT data and substantial computational resources \cite{jiang2024slow1,qin2024o1-replication,xu2025reasoning-survey-rl}. 
% 并且，频繁地切换推理路径容易导致模型遗漏或对表格中的信息产生幻觉，从而出错
% Additionally, frequent transitions between reasoning paths can lead to the model overlooking or hallucinating information in the table, resulting in errors \cite{shi-etal-2024-trusting-Evidence-Hallucinate, Liu2025hallucination-long,zeng2025revisiting-test-truly,yin2025distillation-bottleneck}. 
% 为了解决以上挑战，我们探索training-free的方法，按照指定推理路径迭代推理，来更好地激发模型的表格推理能力
To address these challenges, we explore the training-free method that iteratively guides reasoning along a specified path, aiming to better enhance the table reasoning capabilities, as shown in Figure~\ref{fig:intro}.


% 表格推理任务具有较为规则的结构化evidence，由并列的多行组成，是推理路径的限制和依据
The table reasoning task involves structured evidence, which provides constraints and the basis for reasoning \cite{wang2024chainoftable,ji2024tree-of-table}.
% 所以，本文提出我们的方法，通过提示模型多次逐行遍历表格，激发模型的推理能力
Therefore, we propose \textbf{R}ow-\textbf{o}f-\textbf{T}hought (\ours), which prompts non-reasoning LLMs to perform iterative row-wise table traversals, thereby enhancing their table reasoning capabilities.
% 基于以上的讨论，我们从以下两方面探索
Based on the above discussion, we explore the following two aspects:
% 1. 为了说明我们方法的优越性，我们证明了Long CoT是我们方法的子集
(\emph{i})~To illustrate the superiority of \ours, we discuss that Long CoT is a subset of \ours on the table reasoning task.
% 2. 我们提出了\ours，让non-reasoning LLMs无需训练取得比reasoning LLMs更好的性能
(\emph{ii})~We present \ours, enabling non-reasoning LLMs to achieve superior performance compared to RLLMs without additional training.

% 数学分析和方法
% 为了说明我们方法的优越性，我们首先将我们的方法和Long CoT进行比较
To demonstrate the advantage of \ours, we first compare it with Long CoT. 
% 首先，我们对我们的方法和Long CoT在表格推理任务上进行了数学定义，并分析了二者的函数空间
We begin by providing formal mathematical definitions of \ours and Long CoT within the table reasoning task and analyzing their respective function spaces.
% 通过数学推导证明了Long CoT是我们方法的子集
Through mathematical derivations, we present that the function space of Long CoT is a proper subset of that of \ours.
% 基于以上分析，我们介绍了我们方法的具体做法，模型被提示去多次逐行遍历表格得到最终结果，缓解了Low Reliability和High Cost的限制
Building on the analysis, we detail \ours, where the model is prompted to perform iterative row-wise traversals, to address the limitations of Low Reliability and High Cost.


% 实验
% 为了证明我们方法的有效性，我们在主流数据集WikiTQ, HiTab, TableBench上进行实验
To demonstrate the effectiveness of \ours, we conduct experiments on  WikiTableQuestions~\cite{pasupat-liang-2015-wikitq}, HiTab~\cite{cheng-etal-2022-hitab}, and TableBench~\cite{wu2024tablebench}. 
% 相比较同规模的R1-Distill模型，我们方法未经训练平均提升%，证明了有效性
Compared to Long CoT on RLLMs, \ours achieves an average improvement of $4.3\%$ with non-reasoning LLMs without additional training, validating its effectiveness. 
% 并且，我们在WikiTQ和TableBench上达到了同规模模型的SOTA，在HiTab上也同SOTA可比
Additionally, \ours achieves state-of-the-art (SOTA) results on WikiTableQuestions and TableBench with comparable models, and yields competitive results on HiTab. 
% 分析实验说明了我们方法相较于长思维链模型，以更少的推理token达到了更强的性能
Analysis experiments reveal that \ours outperforms Long CoT with fewer reasoning tokens, showing higher efficiency.
% 并且，我们的方法综合地激发了模型的表格推理能力，包括自主反思能力
% Furthermore, \ours comprehensively enhances the table reasoning capabilities, including the autonomous reflection capability. 

% 我们的贡献如下
Our contributions are as follows:
\begin{enumerate}
    % 1. 我们从数学角度说明了在表格推理任务上多次逐行遍历表格的方法是Long CoT方法的子集
    \item We demonstrate that Long CoT is a subset of iterative row-wise table traversals in the table reasoning task.
    % 2. 我们提出了方法，通过提示模型多次逐行遍历表格，相较于RLLMs有High Reliability和Low Cost的优势
    \item We propose that \ours enables the model to perform iteratively row-wise table traversals, offering advantages of high reliability and low cost compared to RLLMs.
    % 3. 我们在3个主流的表格推理数据集上进行实验，我们的方法平均超过推理模型的性能%,并且在WikiTableQuestions和TableBench上取得了同等规模下的SOTA，证明了有效性
    \item \ours on non-reasoning LLMs outperforms Long CoT on RLLMs by an average of $4.3\%$ and achieves SOTA results among comparable models on WikiTableQuestions and TableBench, proving its effectiveness.
\end{enumerate}




==> old_version/1.introduction_0511.tex <==
% 引出表格推理任务
% 表格推理是一项很重要的任务，其输入包括表格和问题，输出为根据表格对问题的回答
Table reasoning is an important task where the input consists of a question and the table, and the output is the answer based on the table \cite{jin2022table-survey,zhang2025table-survey}. 
% 其中表格由多个并列的行组成，而每行由多个cell组成，包含着大量密集的信息
Tables typically comprise multiple rows, with each row containing several information-dense cells \cite{ruan2024table-data-survey}.
% 由于自动化的表格推理可以帮助人们从表格中抽取出有效信息，提升数据获取效率，收到很多研究者关注
Automated table reasoning attracts considerable research interest due to its potential to extract valuable information from tables, thus accelerating data acquisition \cite{badaro-etal-2023-transformers-table-survey,lu2025table-survey}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{fig/intro.pdf}
    % \vspace{-1.5em}
    \caption{
    % 我们的方法training-free且能更好地激发模型的表格推理能力
    \ours is training-free and can enhance the table reasoning ability better, compared with Long CoT with RLLMs.
    }
    \label{fig:intro}
\end{figure}

% 推理模型及其缺点，引出我们的方法
% 近些年，推理模型凭借引入Long CoT显著提升了模型的推理能力，包括模型的表格推理能力，因为其可以自主规划且切换推理路径，相比较Short CoT浅显且直接的推理
% Long CoT在表格任务上表现为模型可以自主依次选择不同的表格内容进行处理，直到得到最终答案，本文简称为planned order，如图1所示
% 然而，Long CoT在表格推理任务上具备以下缺点
% High Cost: 模型想要获得Long CoT的能力以提升表格推理能力，需要高质量的训练数据，训练成本大
% Low Reliability: planned order的推理路径不一定正确，导致在不同表格内容间切换加剧了模型对相关内容的幻觉或忽视


Recent advancements in reasoning large language models (RLLMs) have significantly enhanced reasoning capabilities utilizing Long Chain-of-Thought (Long CoT), particularly in domains such as mathematics and coding \cite{openai2024openai-o1-card,guo2025deepseek-r1,li202512survey-reasoning}. 
Long CoT refers to autonomously selecting or switching reasoning paths and performing sufficiently deep step-by-step reasoning, in contrast to the shallow and direct reasoning in Short CoT \cite{chen2025reasoning-survey,xu2025redstar,yeo2025demystifying-long-cot}.  
However, current RLLMs exhibit the following limitations:
(\emph{i})~\textbf{Low Reliability}: Frequent transitions between reasoning paths can lead to omissions or hallucinations regarding tabular information, resulting in errors \cite{shi-etal-2024-trusting-Evidence-Hallucinate, Liu2025hallucination-long,zeng2025revisiting-test-truly,yin2025distillation-bottleneck}. 
(\emph{ii})~\textbf{High Cost}: Enhancing table reasoning capabilities of non-reasoning LLMs necessitates high-quality Long CoT data, leading to substantial training expenses \cite{qian2025fino1,jiang2024slow1,qin2024o1-replication}.


% 为了解决以上限制，我们提出Row-of-Thought（\ours），提示模型迭代地逐行处理表格，来增强模型的表格推理能力
% 首先，由于\ours不需要模型自主规划或切换路径，因此我们的方法无需训练，non-reasoning LLM仅根据提示就可以做到
% 并且，\ours指定了模型的推理路径，即严格按照表格原本的行序进行推理，更加符合模型的注意力机制，因此缓解了对表格相关内容的忽视和幻觉
% 基于以上的讨论，我们从两方面证明了\ours的有效性：
% 1. 为了说明\ours中行序的表示能力，我们证明了planned order与行序存在偏序关系
% 2. 我们在3个表格推理的主流数据集上进行实验，\ours with non-reasoning LLMs无需训练取得比reasoning LLMs更好的性能


To address these challenges, we explore the training-free method that iteratively guides reasoning along a specified path, aiming to better enhance the table reasoning capabilities, as shown in Figure~\ref{fig:intro}.
The table reasoning task involves structured evidence, which provides constraints and the basis for reasoning \cite{wang2024chainoftable,ji2024tree-of-table}.
Therefore, we propose \textbf{R}ow-\textbf{o}f-\textbf{T}hought (\ours), which prompts non-reasoning LLMs to perform iterative row-wise table traversals, thereby enhancing their table reasoning capabilities.
Based on the above discussion, we explore the following two aspects:
(\emph{i})~To illustrate the superiority of \ours, we discuss that Long CoT is a subset of \ours on the table reasoning task.
(\emph{ii})~We present \ours, enabling non-reasoning LLMs to achieve superior performance compared to RLLMs without additional training.


% 数学分析和方法
% 为了说明\ours的表示能力，我们首先将行序和planned order进行比较
% 首先，我们将二者看作是数列集合，通过数学推导证明了行序数列比planned order有更强的表示能力
% 具体来说，对于Planned Order中的任意序列，都存在RoT的处理序列，使得前者为后者的子列，因此后者能涵盖前者相同的列和处理顺序

To demonstrate the advantage of \ours, we first compare it with Long CoT. 
We begin by providing formal mathematical definitions of \ours and Long CoT within the table reasoning task and analyzing their respective function spaces.
Through mathematical derivations, we present that the function space of Long CoT is a proper subset of that of \ours.
Building on the analysis, we detail \ours, where the model is prompted to perform iterative row-wise traversals, to address the limitations of Low Reliability and High Cost.


% 实验
% 为了证明我们方法的有效性，我们在主流数据集WikiTQ, HiTab, TableBench上进行实验
To demonstrate the effectiveness of \ours, we conduct experiments on  WikiTableQuestions~\cite{pasupat-liang-2015-wikitq}, HiTab~\cite{cheng-etal-2022-hitab}, and TableBench~\cite{wu2024tablebench}. 
% 相比较同规模的R1-Distill模型，我们方法未经训练平均提升%，证明了有效性
Compared to Long CoT on RLLMs, \ours achieves an average improvement of $4.3\%$ with non-reasoning LLMs without additional training, validating its effectiveness. 
% 并且，我们在WikiTQ和TableBench上达到了同规模模型的SOTA，在HiTab上也同SOTA可比
Additionally, \ours achieves state-of-the-art (SOTA) results on WikiTableQuestions and TableBench with comparable models, and yields competitive results on HiTab. 
% 分析实验说明了我们方法相较于长思维链模型，以更少的推理token达到了更强的性能
Analysis experiments reveal that \textbf{\ours outperforms Long CoT with fewer reasoning tokens, showing higher efficiency}.
% 并且，我们的方法综合地激发了模型的表格推理能力，包括自主反思能力
% Furthermore, \ours comprehensively enhances the table reasoning capabilities, including the autonomous reflection capability. 

% 我们的贡献如下
Our contributions are as follows:
\begin{enumerate}
    % 1. 我们从数学角度说明了在表格推理任务上多次逐行遍历表格的方法是Long CoT方法的子集
    \item We demonstrate that Long CoT is a subset of iterative row-wise table traversals in the table reasoning task.
    % 2. 我们提出了方法，通过提示模型多次逐行遍历表格，相较于RLLMs有High Reliability和Low Cost的优势
    \item We propose that \ours enables the model to perform iteratively row-wise table traversals, offering advantages of high reliability and low cost compared to RLLMs.
    % 3. 我们在3个主流的表格推理数据集上进行实验，我们的方法平均超过推理模型的性能%,并且在WikiTableQuestions和TableBench上取得了同等规模下的SOTA，证明了有效性
    \item \ours on non-reasoning LLMs outperforms Long CoT on RLLMs by an average of $4.3\%$ and achieves SOTA results among comparable models on WikiTableQuestions and TableBench, proving its effectiveness.
\end{enumerate}




==> old_version/1.introduction_0511_1.tex <==
% 引出表格推理任务
% 表格推理是一项很重要的任务，其输入包括表格和问题，输出为根据表格对问题的回答
Table reasoning is an important task where the input consists of a question and the table, and the output is the answer based on the table \cite{jin2022table-survey,zhang2025table-survey}. 
% 其中表格由多个并列的行组成，而每行由多个cell组成，包含着大量密集的信息
Tables typically comprise multiple rows, with each row containing several information-dense cells \cite{ruan2024table-data-survey}.
% 由于自动化的表格推理可以帮助人们从表格中抽取出有效信息，提升数据获取效率，收到很多研究者关注
Automated table reasoning attracts considerable research interest due to its potential to extract valuable information from tables, thus accelerating data acquisition \cite{badaro-etal-2023-transformers-table-survey,lu2025table-survey}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{fig/intro.pdf}
    % \vspace{-1.5em}
    \caption{
    % 我们的方法training-free且能更好地激发模型的表格推理能力
    \ours is training-free and can enhance the table reasoning ability better, compared with Long CoT with RLLMs.
    }
    \label{fig:intro}
\end{figure}

% 推理模型及其缺点，引出我们的方法
% 近些年，推理模型凭借引入Long CoT显著提升了模型的推理能力，包括模型的表格推理能力
Recent advancements in reasoning large language models (RLLMs) have significantly enhanced reasoning capabilities utilizing Long Chain-of-Thought (Long CoT), including table reasoning capabilities \cite{openai2024openai-o1-card,guo2025deepseek-r1,li202512survey-reasoning}. 
% 因为推理模型可以进行深度的推理，自我反思，并探索多样的推理路径，相比较Short CoT浅显且直接的推理
This improvement stems from Long CoT, which performs deep reasoning, engages in self-reflection, and explores diverse reasoning paths, in contrast to the shallow and direct reasoning of Short CoT \cite{chen2025reasoning-survey,xu2025redstar,yeo2025demystifying-long-cot}.
% 然而，现在的推理模型在表格推理任务上具备以下limitation，如图1a所示
However, Long CoT exhibits two limitations in table reasoning, as illustrated in Figure~\ref{fig:intro} (a): 
% High Cost: 模型想要获得Long CoT的能力以提升表格推理能力，需要高质量的训练数据，训练成本大
(\emph{i})~\textbf{High Cost}: Achieving Long CoT capabilities for improved table reasoning capabilities necessitates high-quality data, leading to substantial training expenses \cite{qian2025fino1,jiang2024slow1,qin2024o1-replication}. 
% Low Reliability: 随着输出的推理链条的变长，模型容易丢失输入中的表格信息，造成幻觉
(\emph{ii})~\textbf{Low Reliability}: As the output reasoning chains lengthen, models are prone to losing relevant tabular information from the input, resulting in hallucinations \cite{zhang2023sirens-Hallucination-survey,Liu2025hallucination-long,yin2025distillation-bottleneck,liu2025mathematical-hallucination}. 
% 因此，我们想提出方法，具备Long CoT的优势，同时避免它的限制
Consequently, we aim to propose a method that retains the advantages of Long CoT while mitigating its inherent limitations.



% 所以，我们提出Row-of-Thought（\ours），提示模型迭代地逐行处理表格，来增强模型的表格推理能力，如图1b所示
Therefore, we propose \textbf{R}ow-\textbf{o}f-\textbf{T}hought (\ours), a method that enhances table reasoning by guiding the model to perform iteratively row-wise traversal reasoning, as illustrated in Figure~\ref{fig:intro} (b).
% \ours很好地模拟了Long CoT通过令模型逐行处理表格展开了深度推理
\ours effectively simulates Long CoT by enabling deep reasoning through sequential row-wise traversals. 
% 并且，\ours会在每次遍历表格结束后反思，并选择下一次逐行遍历来推理，直到得到最终答案
Furthermore, \ours incorporates the self-reflection mechanism after each table traversal, selecting the subsequent row-wise traversal accordingly until the final answer is obtained.
% 同时，\ours还具有以下优势
Additionally, \ours offers the following advantages: 
% Low Cost：由于\ours不需要自主探索新的推理路径，因为每条推理路径都按照行序开展，因此我们的方法无需训练，non-reasoning LLM仅根据提示就可以做到
(\emph{i})~Low Cost: Since \ours performs deep reasoning according to the table and the self-reflection capabilities are equipped in non-reasoning LLMs \cite{gu2025survey-judge,ai2025rethinking-reflection-pretraining}, \ours is training-free and can be implemented with non-reasoning LLMs solely through prompting. 
% High Reliability：\ours在推理时强制模型遍历所有行，令模型more attention to表格信息，可以减弱模型的幻觉
(\emph{ii})~High Reliability: By enforcing the sequential traversal of all rows, \ours directs greater attention to tabular information, thereby mitigating hallucination \cite{shi-etal-2024-trusting-Evidence-Hallucinate,chuang2024dola}.



% 实验
% 为了证明我们方法的有效性，我们在主流数据集WikiTQ, HiTab, TableBench上进行实验
To demonstrate the effectiveness of \ours, we conduct experiments on  WikiTableQuestions~\cite{pasupat-liang-2015-wikitq}, HiTab~\cite{cheng-etal-2022-hitab}, and TableBench~\cite{wu2024tablebench}. 
% 相比较同规模的RLLMs，我们方法使用non-reasoning LLMs平均提升%，证明了有效性
Compared to Long CoT on RLLMs, \ours achieves an average improvement of $4.3\%$ with non-reasoning LLMs without additional training, validating its effectiveness. 
% 并且，我们的方法同样可以为推理模型带来进一步性能的提升，缓解了其在表格推理上的幻觉问题
Furthermore, \ours can also enhance the performance of RLLMs with an average improvement of $4.3\%$, mitigating their hallucination issues in table reasoning.
% 此外，我们在WikiTQ和TableBench上达到了同规模模型的SOTA，在HiTab上也同SOTA可比
Additionally, \ours achieves state-of-the-art (SOTA) results on WikiTableQuestions and TableBench with comparable models, and yields competitive results on HiTab. 
% 分析实验说明了\ours相较于长思维链，以更少的推理token达到了更强的性能，因为\ours缓解了推理模型过度思考、内容重复的问题
Analysis experiments reveal that \textbf{\ours outperforms Long CoT with fewer reasoning tokens, showing higher efficiency}, as \ours alleviates issues such as overthinking and content repetition in RLLMs.


% 我们的贡献如下
Our contributions are as follows:
\begin{enumerate}
    % 1. 为了令模型在表格推理任务上获得Long CoT的能力，同时降低成本，我们提出training-free的方法，\ours，which在表格上进行深度推理，并进行反思和探索新推理路径
    \item To equip non-reasoning LLMs with Long CoT capabilities for table reasoning with low costs, we propose a training-free method, \ours, which performs deep reasoning on tables, incorporating reflection and exploration of diverse reasoning paths.
    % 2. 为了解决Long CoT在表格推理上的低可依赖性问题，\ours令模型在推理时逐行遍历表格，以缓解对表格内容的幻觉
    \item To address the low reliability of Long CoT in table reasoning, \ours enables the model to perform iterative row-wise table traverse reasoning, thereby mitigating hallucinations regarding tabular information.
    % 3. 我们在3个主流的表格推理数据集上进行实验，我们的方法平均超过推理模型的性能%,并且在WikiTableQuestions和TableBench上取得了同等规模下的SOTA，证明了有效性
    \item \ours on non-reasoning LLMs outperforms Long CoT on RLLMs by an average of $4.3\%$ and achieves SOTA results among comparable models on WikiTableQuestions and TableBench, proving its effectiveness.
\end{enumerate}






==> old_version/3.methodology_0511.tex <==
% 为了激发语言模型的表格推理能力，我们提出我们的方法
% 正如第二节讨论的，我们提示模型根据多次逐行遍历表格得到最终答案
We propose \ours to enhance the table reasoning ability of non-reasoning LLMs. 
As discussed in \S\ref{sec:analysis} and illustrated in Figure~\ref{fig:method}, \ours guides the model to derive the final answer by performing iterative row-wise traversals of the table. 
The complete prompts are available in Appendix~\ref{app:prompts}.
% 具体来说，我们输入问题Q和表格U，以及提示I和示例D，令模型输出反复遍历表格直到得到答案的过程，如图所示
Concretely, the model is provided with the instruction \( I \), the question \( Q \), the table \( U \), and demonstrations \( D \), and its output is the sequential process of table iteration until the answer is reached.
% 形式化地，C;A = M(Q, U, I, {Q_i, U_i, C_i})
Formally, 
\[
g(Q, U, 0) = M(I, Q, U, \{Q_i, U_i, g(Q_i, U_i, 0)\}),
\]
% 其中，M为语言模型，D = {Q_i, U_i, C_i}，C为推理过程，A为最终答案
where \( M \) is the language model, and \( D = \{Q_i, U_i, g(Q_i, U_i, 0)\} \).
% , \( g \) represents the output of \ours, including the rationale of traversals and the final answer. 
% 我们采用markdown的格式将表格输入模型M中，follow前人工作
We employ the Markdown format to construct the table, following previous works \cite{wang2024chainoftable,zhang2024flextaf,yu2025table-critic}. 
% 我们没有提示模型必须遍历固定次数的表格，而是由模型在推理时根据问题决定
Additionally, we allow the model to decide the number of iterations based on the question during reasoning without a fixed number of traversals.
This capability, where the model self-regulates the traversal count during inference, is exemplified in Figure~\ref{fig:traversal_num}.
% 因为我们发现模型具备在推理时自主决定遍历次数的能力，如图b所示
% This is because we observe that the model can autonomously determine the necessary number of traversals during inference, as illustrated in Figure B. 
% 我们在4.3节详细分析什么时候模型需要多次遍历才能得到答案
Further elaboration on the circumstances necessitating multiple traversals is listed in \S\ref{subsub:table traversal counts}.

==> old_version/3.methodology_0515.tex <==
% 为了缓解Long CoT的High Cost and Low Reliability的限制，我们提出training-free的方法\ours
To mitigate the limitations of High Cost and Low Reliability in Long CoT, we propose a training-free method, \ours. 
% 如图所示，\ours通过令模型迭代逐行遍历表格增强表格推理能力
As illustrated in Figure~\ref{fig:method}, \ours enhances table reasoning capabilities by enabling the model to perform iterative row-wise traversals.
% 完整的prompt在附录中提供
The complete prompts are available in Appendix~\ref{app:prompts}.
% 我们输入提示I，问题Q和表格U，以及示例D，模型输出迭代逐行遍历表格直到得到答案的过程
Given an instruction $I$, a question $Q$, a table $U$, and in-context demonstrations $D$, the model outputs a step-by-step reasoning process that iteratively traverses the table in the sequential row order until the final answer is derived.
% 形式化地，R;A = M(Q, U, I, {Q_i, U_i, R_i, A_i})，其中，M为语言模型，D = {Q_i, U_i, R_i, A_i}，R为推理过程，A为最终答案
Formally, $R;A = \mathcal{M}(Q, U, I, \{Q_i, U_i, R_i, A_i\})$, where $\mathcal{M}$ is the LLM, $D = \{Q_i, U_i, R_i, A_i\}$, $R$ represents the reasoning process, and $A$ is the final answer. 
% 我们采用markdown的格式表示表格，follow前人工作
We represent the table in Markdown format, following previous works \cite{wang2024chainoftable,zhang2024flextaf,yu2025table-critic}. 
% 下面我们分别介绍在\ours的推理过程$R$中的两个重要因素


\subsection{Traversal}
% 我们首先介绍\ours中逐行遍历的过程
% 

\subsection{Iteration}
% 具体地说，模型每步根据问题和之前的推理对表格当前行的内容进行推理，直到遍历完整的表格
Specifically, at each step, the model reasons about the content of the current row based on the question and the preceding reasoning until the entire table has been traversed.
% 迭代地遍历具体表现为每次遍历结束，模型可以选择继续推理，因为涉及多行依赖或多跳的问题无法在一次遍历中得到答案
This iterative process allows the model to continue reasoning after a traversal, which is necessary for multi-hop questions that cannot be answered in a single traversal.
% 模型也可以选择在遍历结束后对之前的推理进行反思，并根据反思的内容重新遍历表格直到得到最终答案
The model can also choose to reflect on the previous reasoning after a traversal and subsequently revisit the table based on the reflection until the final answer is obtained.
% 我们没有固定模型遍历表格的次数，而是由模型在推理时自主决定，如图显示
Instead of predefining the number of traversals, the model autonomously decides when to stop during inference, as shown in Figure~\ref{fig:traversal_num}.
% 我们在4.3节详细分析了模型多次遍历表格的情况
We provide a detailed analysis of the iterative table traversal scenarios in \S\ref{subsub:table traversal counts}.





==> old_version/4.experiment_0512.tex <==
\subsection{Experimental Setup}
\paragraph{Dataset}
% 我们follow前人工作，使用WikiTableQuestions, HiTab和TabelBench的popular表格推理数据集上评测我们方法的性能
\ours is evaluated on three widely used table reasoning datasets: WikiTableQuestions~\cite{pasupat-liang-2015-wikitq}, HiTab~\cite{cheng-etal-2022-hitab}, and TableBench~\cite{wu2024tablebench}, following previous works \cite{zhao-etal-2023-parser,jiang2024sscot,cao2025tablemaster,li-etal-2025-graphotter}. 
% WikiTQ是表格推理的主流表格QA数据集，需要模型根据表格回答问题
WikiTableQuestions is a mainstream table-based question answering dataset that requires models to reason over tabular content.
% HiTab关注于hierarchical表格，对模型理解表格展现出挑战
HiTab focuses on hierarchical tables, challenging models to comprehend complex structural relationships.
% TableBench是综合的、具有挑战的数据集，包含多样的问题类型和topic
TableBench presents a comprehensive and challenging benchmark covering diverse question types and topics.

\paragraph{Models}
% 对于语言模型，我们采用Llama3.1-8B-Instruct (Llama3.1-8B), Llama3.3-70B-Instruct (Llama3.3-70B)，Qwen2.5-7B-Instruct (Qwen2.5-7B)和Qwen2.5-32B-Instruct (Qwen2.5-32B)
For non-reasoning LLMs, we utilize Llama3.1-8B-Instruct (Llama3.1-8B), Llama3.3-70B-Instruct (Llama3.3-70B) \cite{dubey-etal-2024-llama3.1}, Qwen2.5-7B-Instruct (Qwen2.5-7B), and Qwen2.5-32B-Instruct (Qwen2.5-32B) \cite{yang2024qwen25}. 
% 对于推理模型，我们采用对应规模的DeepSeek-R1-Distill-Llama-8B (R1-Llama-8B), DeepSeek-R1-Distill-Llama-70B (R1-Llama-70B), DeepSeek-R1-Distill-Qwen-7B (R1-Qwen-7B)和DeepSeek-R1-Distill-Qwen-32B (R1-Qwen-32B)
For RLLMs, we employ the corresponding-sized DeepSeek-R1-Distill-Llama-8B (R1-Llama-8B), DeepSeek-R1-Distill-Llama-70B (R1-Llama-70B), DeepSeek-R1-Distill-Qwen-7B (R1-Qwen-7B), and DeepSeek-R1-Distill-Qwen-32B (R1-Qwen-32B) \cite{guo2025deepseek-r1}. 
% 其中，我们没有采用DeepSeek-R1-Distill-Qwen-7B的base model Qwen2.5-Math-7B，是因为这一模型主要适用于数学任务，在表格推理任务上的性能较差
We exclude Qwen2.5-Math-7B, which is the base model of DeepSeek-R1-Distill-Qwen-7B, due to its primary focus on solving mathematical tasks, resulting in suboptimal performance on table reasoning tasks \cite{yang2024qwen25-math}.

\paragraph{Metric}
% 对于WikiTableQuestions和HiTab，我们采用准确率作为评价指标，follow前人工作
For WikiTableQuestions and HiTab, we adopt accuracy as the evaluation metric, following prior works \cite{pasupat-liang-2015-wikitq,cheng-etal-2022-hitab}. 
% 准确率衡量了模型生成和gold answer完全匹配的答案的能力
Accuracy measures the ability of models to generate answers that exactly match the gold answers. 
% 对于TableBench，我们采用Rouge-L，follow前人工作
For TableBench, we use Rouge-L~\cite{lin-2004-rouge}, consistent with the previous research \cite{wu2024tablebench}. 
% Rouge-L通过最长公共子序列衡量模型生成的答案的质量，兼顾考虑了Precision和Recall
Rouge-L evaluates the quality of generated answers based on the longest common subsequence, considering both precision and recall.


\paragraph{Baselines}
% 对于我们的方法，我们采用one-shot的prompt，为了令模型详细了解如何逐行遍历表格
\ours employs a one-shot prompt to enable \textbf{non-reasoning LLMs} and \textbf{RLLMs} to perform iterative row-wise table traversals (prompts in Appendix~\ref{app:prompts}). 
% 因此，我们将我们的方法和以下方法进行比较
We compare \ours with the following methods:
\begin{itemize}
    % CoT with language model （one-shot）：我们采用了和我们方法相同的示例，提示语言模型think step by step再输出答案
    \item Short CoT: We apply the same demonstration as \ours, prompting \textbf{non-reasoning LLMs} to engage in step-by-step reasoning.
    % CoT with reasoning model （zero-shot）：我们提示推理模型回答问题。由于我们采用的推理模型不具备in-context learning的能力，加上示例反而会带来性能的下降（见附录），所以我们采用zero-shot的prompt
    \item Long CoT: We utilize the zero-shot prompt for the corresponding \textbf{RLLMs}, because of the observed performance degradation with in-context learning for the employed RLLMs \cite{guo2025deepseek-r1,zheng2025curse-cot-limitations-icl} (refer to Appendix~\ref{subapp:Long CoT with few-shot prompt})
    % 其他表格推理的前人工作：我们在附录将我们的方法和先进的前人工作比较
    \item Previous table reasoning works: A comprehensive comparison with existing table reasoning methods is presented in Appendix~\ref{subapp:Comparison with previous methods}.
\end{itemize}


\begin{table*}[t]
    \centering
    \small
    \input{tab/main}
    \caption{ 
        % 我们的方法和基线的性能对比
        Performance comparison between \ours and baselines.
        % WikiTQ指WikiTableQuestions
        WikiTQ refers to WikiTableQuestions.
        % $\Delta$代表我们的方法相比推理模型的性能的增涨
        $\Delta$ denotes the performance improvement of \ours over the reasoning models.
    }
    \label{tab:main}
\end{table*}

\begin{table}[t]
    \centering
    \small
    \input{tab/SOTA_comparison}
    \caption{ 
        % 我们的方法和基线的性能对比
        Performance comparison between \ours and SOTA methods with similar scale models on three datasets.
    }
    \label{tab:SOTA_comparison}
\end{table}


\subsection{Main Results}
% 表1展现了我们的方法使用不同模型在不同数据集上和基线的对比
Table~\ref{tab:main} presents a comparison between \ours and baselines using different models across various datasets.
% 可以发现，我们的方法一致且显著地超越了推理模型的性能，平均提升%
\ours, using non-reasoning LLMs consistently and significantly outperforms Long CoT with RLLMs, achieving an average improvement of $4.3\%$, demonstrating its effectiveness.
% 并且，我们的方法能为推理模型带来进一步的提升，平均提升3%，
% 我们还发现
We also observe that:

\paragraph{Baselines}
% 我们的方法超越Long CoT，一方面是因为正如第二节讨论的，数学上我们的方法更包含Long CoT，一方面是因为我们固定了推理路径必须按照表格行序遍历，避免了Long CoT因为频繁变换推理路径导致遗漏相关信息的问题
\ours outperforms Long CoT because Long CoT is mathematically a subset of \ours, as discussed in \S\ref{sec:analysis}.
Furthermore, by fixing the reasoning path to follow the table row order, \ours mitigates the issue in Long CoT where frequent reasoning path changes can lead to the omission of relevant information.
% 而我们的方法能够超越Short CoT，是因为它逐行遍历表格进行细粒度推理，降低了每一步的推理难度，而且不容易遗漏相关信息
Compared to Short CoT, \ours achieves superior performance through fine-grained, row-wise reasoning, thereby reducing the complexity of individual reasoning steps and minimizing the risk of overlooking relevant details.

% 并且，我们将我们的方法和前人方法在WikiTQ和HiTab上进行比较，如表2和表3所示
We also compare \ours with SOTA methods on three datasets, as shown in Table~\ref{tab:SOTA_comparison}.
% 受限于空间，我们在附录详细介绍SOTA方法，并将我们的方法和更多前人工作比较
Due to space constraints, detailed comparisons with prior works are provided in Appendix~\ref{subapp:Comparison with previous methods}.
% 可以发现，我们的方法超过了使用同等规模甚至更大模型的前人工作的性能，进一步证明了我们方法的有效性
\ours outperforms previous works on WikiTQ and TableBench and is comparable with the SOTA method on HiTab, highlighting its effectiveness.
% 我们的方法没有像前人方法那样专门根据嵌套表格进行改进，所以没有在HiTab上也达到SOTA
The comparable performance on HiTab can be attributed to the fact that \ours does not incorporate specific enhancements for hierarchical tables, unlike previous methods \cite{zhao-etal-2023-parser,jiang2024sscot,li-etal-2025-graphotter}.

\paragraph{Models}
% 我们的方法在不同规模的模型上均得到显著提升，且均超过对应推理模型的性能
\ours consistently demonstrates substantial performance improvements across models of varying scales, outperforming their corresponding RLLMs.
% 同时，R1-Qwen-7B在HiTab上的性能未超过Qwen2.5-7B，因为R1-Qwen-7B的Base model是Qwen2.5-Math-7B，which主要用于解决数学问题，不同于其他模型的base model是general models
Additionally, R1-Qwen-7B does not outperform Qwen2.5-7B on HiTab, as its base model, Qwen2.5-Math-7B, is optimized for mathematical reasoning, unlike the general-purpose base models of others \cite{yang2024qwen25-math}.


\paragraph{Datasets}
% 我们的方法在HiTab上的提升相较于其他数据集上的提升更显著
\ours yields more pronounced improvements on HiTab compared to other datasets. 
% 因为模型对于嵌套表格的理解比较困难，而我们的方法通过逐行遍历更加细节地理解了表格
This can be attributed to the greater complexity of hierarchical tables for table understanding, where our row-wise traversal facilitates a more fine-grained comprehension of table structure and content. 

\subsection{Analysis Experiments}
% 我们主要选取Llama3.1-8B进行后续分析实验，受限于篇幅
We primarily select Llama3.1-8B for subsequent analysis experiments due to its high reasoning efficiency and space limitations. 

\begin{figure}[t]
\centering
\input{fig/error}
\vspace{-0.5em}
\caption{
    % Long CoT因为呈现出的错误类型而不如\ours
    Long CoT underperforms \ours due to the error types, with their distribution.
}
\label{fig:error}
\end{figure}

\subsubsection{Why \ours Outperforms Long CoT?}
% 为了更具体地分析为什么我们方法的性能超过Long CoT，我们随机选取了我们的方法使用Llama3.1-8B在WikiTQ上的做对，但Long CoT使用R1-Llama-8B没做对的instance，手动分析了原因，比例如图所示
To explore the superior performance of \ours over Long CoT, we conduct an error analysis on WikiTQ instances where \ours with Llama3.1-8B succeeds while Long CoT with R1-Llama-8B fails. Figure~\ref{fig:error} illustrates the identified error categories on sampled $50$ instances, which are detailed below:


% Hallucination指的是模型记错了表格中的信息，出现在推理中的表格内容和输入的不一致，比如混淆了不同行的内容
(\emph{i})~\textbf{Hallucination} refers to the model incorrectly recalling table information, leading to inconsistencies between the table input and the generated reasoning.
% , such as cross-row confusion. 
% Long CoT这种现象如此严重，因为频繁转换推理路径，在不同位置的cell间跳转加剧了对输入信息的遗忘进而幻觉
Long CoT exhibits a higher frequency of hallucinations, due to its frequent shifts in reasoning paths, which cause the model to forget input details \cite{Liu2025hallucination-long}. 
% 而我们的方法按照行序顺序遍历，符合注意力机制，减轻了这种现象
Conversely, \ours performs row-wise traversals in order, aligning with the attention mechanism, which mitigates this issue \cite{yin-etal-2020-tabert,badaro-etal-2023-transformers-table-survey}.
% Overlooking指的是模型没有关注到表格中的问题相关信息
(\emph{ii})~\textbf{Overlooking} refers to failing to focus on the relevant information in the table. 
% 由于Long CoT的推理顺序较为自由，在不同位置的cell间跳转很容易没有覆盖到所有表格，进而忽视了相关内容
The flexible reasoning order and frequent transitions between cells in Long CoT increase the susceptibility to overlooking crucial data.
% 而我们的方法要求遍历表格所有内容，减轻了这种现象
In contrast, \ours requires a complete traversal of the table, thus alleviating this issue.
% Misunderstanding指的是模型由于误解问题而产生错误的推理，这是蒸馏模型带来的问题
(\emph{iii})~\textbf{Misunderstanding} denotes the misinterpretation of the question, which is a common challenge for distilled models \cite{banerjee2024llms-hallucinate-live,yin2025distillation-bottleneck}.
% Linking指的是模型根据问题定位到了表格中错误的位置
(\emph{iv})~\textbf{Linking} refers to incorrectly identifying the relevant table location for the given question. 
% 说明我们的方法很好地激发了模型的表格推理能力，包括对问题的分析能力和对表格的理解能力
The reduced occurrence of the last two errors suggests that \ours effectively enhances table reasoning capabilities, including question understanding and table comprehension.


\begin{figure}[t]
\centering
\input{fig/multi_traversal}
\caption{
    % 我们的方法遍历多次表格的原因，及其比例
    The distribution of reasons for iterative traversals in \ours on sampled $60$ instances from three datasets.
}
\label{fig:multi_traversal}
\end{figure}

% \begin{figure*}[htbp]
% \centering
% \input{fig/traversal_num}
% \caption{
%     % 在3个数据集上，我们方法遍历表格次数的分布和相应的性能
%     The distribution of table traversal counts and the corresponding performance of \ours on three datasets.
% }
% \label{fig:traversal_num}
% \end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=1\linewidth]{fig/traversal_num.pdf}
\vspace{-2.0em}
\caption{
    % 在3个数据集上，我们方法遍历表格次数的分布和相应的性能
    The distribution of table traversal counts and the corresponding performance of \ours on three datasets.
}
\label{fig:traversal_num}
\end{figure*}

\subsubsection{How does table traversal count affect \ours?}
\label{subsub:table traversal counts}
% 为了分析我们的方法何时需要多次遍历表格，我们分别从3个数据集随机抽取了20条我们方法大于一次地遍历表格的数据并分析其多次遍历的原因，如图所示
To examine when \ours requires iterative traversals, we randomly select $20$ instances from each dataset where \ours traverses the table multiple times and investigate the underlying reasons, as shown in Figure~\ref{fig:multi_traversal}. 
% 我们首先详细介绍这3个多次遍历的原因，对应的例子见附录
We first provide a detailed explanation of the three reasons, with examples provided in Appendix~\ref{subapp:Case study of ours with iterative traversals}.
% 1. Multi-Step Reasoning：问题本身需要多次遍历表格才能解决，比如跨行依赖等
(\emph{i})~\textbf{Multi-Step Reasoning}: The inherent complexity of certain questions demands iterative table traversals to derive the solution, particularly when addressing cross-row dependencies.
% 2. Reflection：令人意外的是，即使我们没有提示模型反思自己的推理，但模型依然自发地表现出自我反思的行为。这也进一步说明了我们方法可以综合地激发模型的表格推理能力。
(\emph{ii})~\textbf{Reflection}: Notably, even without explicit prompting for reflective reasoning, the model spontaneously exhibited self-reflection.
% 这表明非推理模型也存在self-reflection的能力，而我们的方法综合地激发了模型的表格推理能力，包括self-reflection的能力
This observation suggests an inherent capacity of self-reflection even in non-reasoning LLMs \cite{ai2025rethinking-reflection-pretraining}, and \ours effectively elicits comprehensive table reasoning capabilities, including this self-reflective ability.
% 3. Summary：在进行必要的推理后，重新遍历表格总结答案。
(\emph{iii})~\textbf{Summarization}: Following the necessary reasoning steps, the model re-traverses the table to generate a concise summary of the answer.



% 并且为了分析遍历次数对我们方法的影响，我们统计了在使用Llama3.1-8B时遍历表格次数的分布以及对应的性能，如图所示
Additionally, to assess the impact of traversal count on performance, we report the distribution of table traversal counts and the corresponding performance when using Llama3.1-8B, as depicted in Figure~\ref{fig:traversal_num}.
% 观察图3，我们发现
We observe that:
% 1. 即使我们没有显式提示模型遍历几次表格，但模型会按需遍历多次。在更具有挑战性的TableBench上我们的方法倾向于遍历次数更多
(\emph{i})~On the more challenging TableBench dataset, \ours tends to perform more traversals as required.
% 2. 随着遍历次数的增多，我们方法的性能下降。因为一方面需要多次遍历的问题本身更难，一方面多次遍历表格容易造成在得到最终答案之前超出token限制
(\emph{ii})~Increasing traversal counts correlate with a decrease in the performance of \ours, due to the inherent difficulty of questions necessitating iterative traversals and the potential for exceeding token limits during such processes.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{fig/token_num.pdf}
    \vspace{-2.0em}
    \caption{
    % 在3个数据集上，我们方法和基线正确推理平均长度和错误的推理平均长度的对比
    Comparison of average reasoning lengths for correct and incorrect inferences across three datasets.
    }
    \label{fig:token_num}
\end{figure*}

% 推理token的统计
\subsubsection{How does reasoning length affect table reasoning capabilities?}
% 为了探索推理长度对表格推理性能的影响，我们分别统计了不同方法的正确推理平均长度和错误的推理平均长度，如图所示
To investigate the impact of reasoning length on table reasoning performance, we calculate the average number of tokens used in correct and incorrect reasoning on each dataset, as shown in Figure~\ref{fig:token_num}. 
% 可以发现
The results reveal that:
% 1. 我们的方法使用较少的token实现了表格推理能力的提升
(\emph{i})~\ours outperforms Long CoT in table reasoning with fewer tokens.
% 因为整体上我们方法的推理长度长于Short CoT，短于Long CoT，且我们的方法性能最好
Specifically, the average reasoning length of \ours lies between that of Short CoT and Long CoT, yet it achieves the highest overall performance.
% 一方面，因为逐行遍历表格能够更细粒度地推理，而且减少了遗漏相关信息的风险
This can be attributed to two factors. 
First, row-wise table traversals facilitate more granular reasoning and mitigate the risk of overlooking pertinent information.
% 另一方面，我们使用的模型没在长推理数据上专门训练过，可以按照问题需求灵活变化推理长度
Second, non-reasoning LLMs are not explicitly trained on Long CoT data, enabling them to adapt the reasoning length flexibly based on question complexity.
% 2. inference-time scale可以激发模型的表格推理性能，但过多的推理token也会带来性能下降。
(\emph{ii})~Inference-time scaling can enhance the table reasoning capability, however, excessive reasoning tokens lead to performance degradation. 
% Long CoT错误的推理长度格外的长，说明了频繁切换推理路径容易导致遗漏表格中的相关信息，并且过度思考、内容重复、错误累积等现象严重
The notably longer reasoning length observed in incorrect predictions of Long CoT suggests that frequent transitions between reasoning paths can result in the hallucination and omission of relevant table information \cite{he2025detect-errors,arcuschin2025CoT-not-Faithful,yin2025distillation-bottleneck}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{fig/table_size.pdf}
    \vspace{-2.0em}
    \caption{
    % 在3个数据集上，我们方法和基线在不同表格尺寸上平均性能的比较
    The comparison of the average performance of \ours and baselines on different table sizes.
    }
    \label{fig:table_size}
\end{figure*}

% 我们的方法随着表格尺寸的变化如何变化
\subsubsection{How does \ours change with table size?}
% 为了分析我们的方法在不同表格尺寸上的性能变化，我们比较了我们的方法和基线使用Llama3.1-8B在不同表格尺寸上的性能，其中表格尺寸是表格行数和列数的乘积，如图所示
To evaluate the performance of \ours relative to baselines across varying table sizes, we analyze the performance of Llama3.1-8B on tables of different sizes, defined as the product of the number of rows and columns (Figure~\ref{fig:table_size}).
% 可以发现
The key observations are as follows:
% 1. 我们的方法在不同尺寸上的性能整体上优于基线
(\emph{i})~Overall, \ours outperforms the baselines across table sizes.
% 2. 我们的方法随着表格尺寸变大，性能变化较为稳定，但整体呈现下降趋势
(\emph{ii})~While exhibiting a general downward trend, the performance of \ours demonstrates relative stability with increasing table size.
% 我们的方法由于需要逐行遍历表格进行细粒度的推理，表格行数过多容易在还未得到答案时超出token限制
The row-wise processing of \ours can lead to exceeding the token limit when the number of rows becomes excessively large before a response is generated.
% 而推理模型由于表格尺寸较大，推理步骤和推理路径增多，也容易超出token限制
Long CoT suffers from an increased number of reasoning steps and pathways with larger tables, elevating the risk of overlooking or hallucinating relevant information and surpassing token limits \cite{zeng2025revisiting-test-truly,sui2025overthinking-survey}.
% 而普通CoT的方法虽然不容易超出token限制，但推理的粒度过大，容易遗漏或找错相关的表格内容
Conversely, Short CoT, while less susceptible to token limit issues, may omit or misinterpret relevant table content due to its coarser reasoning granularity \cite{snell2024scaling-test-time,zhang2025why-cotprompt-not-work}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{fig/unit_performance.pdf}
    \vspace{-2.0em}
    \caption{
    % 在3个数据集上，我们方法使用不同遍历单位的性能比较
    Comparison of \ours traversing the table with different units across three datasets.
    }
    \label{fig:unit_performance}
\end{figure*}

% 不同单位的遍历方法
\subsubsection{How does the traversal unit affect \ours?}
% 为了探索遍历单位对我们方法的影响，我们分别采用行、列和cell使用Llama3.1-8B进行实验，结果如图所示
To investigate the effect of traversal units on \ours, we conduct experiments using rows, columns, and individual cells as traversal units across three datasets with Llama3.1-8B.
% 其中，逐行遍历是我们主实验采用的单位
Row-wise traversal is adopted as the default setting in the main experiments.
% 结果显示
The results indicate the following:

% 1. 在WikiTQ和TableBench上我们的方法都是以行为单位的性能最高
(\emph{i})~On WikiTQ and TableBench, row-wise traversal achieves the best performance. 
% 因为相比按列遍历，逐行遍历更符合模型的注意力机制，便于模型将注意力集中在同一行的各个单元格上
Compared to column-wise traversal, row-wise traversal better aligns with the attention mechanism, enabling more effective focus on all cells within the same row \cite{yin-etal-2020-tabert,liu-etal-2024-rethinking-tabular}. 
% 而按cell遍历性能下降显著，是因为按cell遍历的推理粒度过于小，且大量的cell是问题无关的，冗余的推理步骤增加了误差累积的风险
Cell-wise traversal resulted in a significant performance decrease, due to its overly fine-grained reasoning granularity and the presence of numerous irrelevant cells, which introduce redundant reasoning steps and increase the risk of error accumulation \cite{jin-etal-2024-impact-Reasoning-Step,chen2024Boundary}.
% 2. 相反，在HiTab上我们的方法按列遍历的性能最好
(\emph{ii})~Column-wise traversal yields superior performance on HiTab. 
% 考虑到HiTab中的cell可能对应多个嵌套的header，逐行遍历时需要对应每个cell的内容到多个header，而逐列遍历时header的信息已经包含到这一列中了，所以按列遍历的性能更好
% HiTab中所有的表格都具有hierarchical row headers，93.1%的表格具有hierarchical column headers，相对较少
In HiTab, all tables include hierarchical row headers, while hierarchical column headers are present in $93.1\%$ of the tables, a relatively less frequent occurrence \cite{cheng-etal-2022-hitab}. 
% 因此，其中每行都每个cell都对应hierarchical row headers，逐行遍历时需要对应每个cell的内容到多个row headers，而逐列遍历时header的信息已经包含到这一列中了，所以按列遍历的性能更好
Consequently, each cell in a row corresponds to hierarchical row headers. 
During row-wise traversals, each cell should be mapped to multiple row headers, whereas column-wise traversals inherently incorporate header information into each column, facilitating more effective reasoning \cite{zhao-etal-2023-parser}.


\begin{figure}[ht]
\centering
\input{fig/shot_num}
\vspace{-0.5em}
\caption{
    % 我们的方法在WikiTQ上随着示例数量变化的性能
    Performance of \ours on WikiTQ with varying numbers of demonstrations.
}
\label{fig:shot_num}
\end{figure}

% 示例数量对我们方法的影响
\subsubsection{How does the number of demonstrations affect \ours?}
% 为了探索示例数量对我们方法的影响，我们在WikiTQ上使用Llama3.1-8B进行实验，结果如图所示
To investigate the effect of the number of demonstrations on \ours, we conduct experiments on WikiTQ using Llama3.1-8B, as illustrated in Figure~\ref{fig:shot_num}. 
% 具体地，我们的示例均选取于WikiTQ的训练集
All demonstrations were sampled from the WikiTQ training set.
% 我们发现
We observe that:
% 1. 示例数量从0变化到1时，性能上升最为明显
(\emph{i})~A substantial performance gain is observed when transitioning from zero-shot to one-shot prompting. 
% 因为示例有利于模型理解指令，并且可以根据示例中的推理过程模仿如何遍历表格得到答案，更好地激发了模型的表格推理能力
This suggests that a single demonstration significantly aids the model in comprehending the instruction and replicating the reasoning process for table traversal and answer derivation, thus improving table reasoning capabilities.
% 2. 随着示例数量的增多，性能先上升后下降
(\emph{ii})~With a further increase in the number of demonstrations, performance initially improves but subsequently declines.
% 因为少量示例已经令模型很好地理解指令，学会逐行推理，更多的示例很难带来更多知识上的增益，反而容易限制模型的推理路径
A limited number of demonstrations is sufficient for the model to understand the instructions and learn the reasoning patterns. 
Additional demonstrations contribute little new information and may constrain the reasoning paths \cite{lin2024Alignment-icl,wan2025many-shot,zheng2025curse-cot-limitations-icl}.
% 因此，在主实验中我们选取了one-shot prompt，为了平衡了推理性能和效率
Therefore, we employ the one-shot prompt in the main experiments to achieve a balance between inference performance and efficiency.




==> tex/2.analysis.tex <==
\subsection{Problem Formulation}
% 首先，我们对我们问题的输入和输出进行定义
First, we formally define the input and output spaces for the table reasoning task.
% 令 $\mathbb{U} \subseteq \mathbb{R}^{d \times N \times M}$ 表示输入矩阵空间，其中 $d, N, M \in \mathbb{R}$ 分别表示每个 cell 对应的嵌入向量的维度、矩阵的行和列。令 $\varnothing \in \mathbb{U}$ 表示空矩阵（即不提供表格信息），$U = \left\{ u_{1}, \ldots, u_{m} \right\}$ 表示单个矩阵，其中 $u \in \mathbb{R}^{d \times N}$ 表示矩阵的每一行。
The input table space is denoted as \(\mathbb{U} \subseteq \mathbb{R}^{d \times N \times M}\), where \(d \in \mathbb{N}\) represents the embedding dimension of each table cell, and \(N, M \in \mathbb{N}\) are the number of rows and columns, respectively. 
Specifically, the absence of table information is represented by the empty matrix \(\varnothing \in \mathbb{U}\). A single table \(U = \{u_1, \ldots, u_m\}\) consists of \(m\) row vectors \(u_i \in \mathbb{R}^{d}\). 
% 令 $\mathbb{V} \subseteq \mathbb{R}^{d}$ 表示用户问题和输出的向量空间，$Q \in \mathbb{V}$ 表示用户问题。
The semantic vector space of user questions and outputs is defined as \(\mathbb{V} \subseteq \mathbb{R}^{d}\), where \(Q \in \mathbb{V}\) denotes the natural language question. 
% 令 $S = \left\{ s \right\} \subseteq \mathbb{R}^{d}$ 表示累计的信息，$0$ 表示空信息量。
The cumulative information state \(S = \{s\} \subseteq \mathbb{R}^{d}\) stores contextual information, with the initial empty state being \(0 \in \mathbb{R}^{d}\).
% 令 $f \in \left( \mathbb{R} \times \mathbb{U} \right) \to \mathbb{V}$ 表示一个计算映射。
% Let \(f \in (\mathbb{R} \times \mathbb{U}) \to \mathbb{V}\) represent a computational mapping.
 

% 我们方法的定义
\paragraph{Definition of \ours}
% 我们的方法通过多次逐行遍历表格得到最终答案
\ours formalizes table reasoning as an iterative state transition system, performing sequential row-wise traversals to derive the final answer.
% 即作为一个状态转移函数，每次接受问题和表格，根据上一个状态接受的表格行，基于顺序的下一行或者下一次遍历的第一行进行推理
Specifically, at each step, given a question \(Q\) and a table \(U\), \ours reasons over either the subsequent row or the first row of the next traversal pass, conditioned on the previous state. 
% 形式化地我们的方法作为映射集合$\mathcal{R} \subseteq \left( \mathbb{R} \times \mathbb{U} \times \mathbb{S} \right) \to \mathbb{V}$$，满足： 
Formally, \ours is defined as a set of mappings \(\mathcal{R} \subseteq (\mathbb{R} \times \mathbb{U} \times \mathbb{S}) \to \mathbb{V}\), subject to the following conditions:
\begin{equation}
h_{0} \in \mathcal{R},\ \text{s.t.}\ h_{0}(Q, \varnothing, 0) = Q
\end{equation}
\begin{equation}
\begin{aligned}
h \in \mathcal{R},\ \text{s.t.}\ &h(Q, U, 0) = \\
&h\left( Q, \left( u_{M} \right), h\left( Q, U / u_{M}, 0 \right) \right)
\end{aligned}
\end{equation}
% 其中，u_m为表格的最后一行，则我们的方法
where \(u_{M}\) is the last row of the table \(U\). 
So the complete reasoning process of \ours is defined as, for \(\forall h \in \mathcal{R},\ Q \in \mathbb{R}^{d},\ U \in \mathbb{U}\):
\begin{equation}
\begin{aligned}
g(Q, U, 0) = g\left( Q, U, h(Q, U, 0) \right) \in \mathcal{R},\\
\end{aligned}
\end{equation}


\paragraph{Definition of Long CoT}
% 结合前人对Long CoT的定义，并结合表格推理任务，Long CoT在表格推理任务上可以看作是一个状态转移函数，每次根据问题和表格中的某些信息进行下一步操作，这类操作可能包括顺序推理、反思、探索另一条推理路径等
Building upon prior definitions of Long CoT and focusing on table reasoning, we conceptualize Long CoT as a state transition function \cite{zhang2024auto-regressive-cot,zhang2025finite-state-automata-transformers}. 
At each step, it executes an operation conditioned on the question and relevant table information, encompassing sequential reasoning, reflection, and exploration of alternative reasoning paths \cite{chen2025reasoning-survey,xu2025redstar,yeo2025demystifying-long-cot}.
% 我们在这里采用row作为状态转移输入单位，并在附录中讨论了采用其他单位的Long CoT定义以及后续的证明
We adopt the row as the unit for state transition inputs, and discuss Long CoT with other units and subsequent discussion in Appendix~\ref{app:unit selection}.
% 形式化地，Long CoT作为映射空间的集合 $\mathcal{L} \subseteq \left( \mathbb{R} \times \mathbb{U} \right) \to \mathbb{V}$，满足：
Formally, Long CoT is defined as a set of mappings within the space \(\mathcal{L} \subseteq (\mathbb{R} \times \mathbb{U} \times \mathbb{S}) \to \mathbb{V}\), satisfying the following conditions:
\begin{equation}
\begin{aligned}
f_{0} \in \mathcal{L},\ \text{s.t.}\ f_{0}(Q, \varnothing, 0) = Q
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
&f \in \mathcal{R}, \exists i \in \left\{ 1, \ldots, M \right\},\\
& \ \text{s.t.}\ f(Q, U, 0) = f\left( Q, \left\{ u_{i} \right\}, f\left( Q, U / u_{i}, 0 \right) \right),\ 
\end{aligned}
\end{equation}


\subsection{Long CoT is the subset of \ours}
% 在本小节我们证明Long CoT的映射集合是我们方法的子集，通过将我们的方法对齐到Long CoT
In this subsection, we discuss that the mapping set of Long CoT is a subset of \ours by aligning our method to Long CoT in the specific conditions.
% 对于任意 $f \in \mathcal{L}$，任意 $Q, U$，记 $\sigma_{i}$ 满足：
For $\forall f \in \mathcal{L}$, $\forall Q, U$, let $\sigma_{i}$ satisfy:
\begin{equation}
\begin{aligned}
&f\left( Q, U / \{ u_{\sigma_{1}}, \ldots, u_{\sigma_{i - 1}} \}, 0 \right) = \\
&f\left( Q, \left\{ u_{\sigma_{i}} \right\}, f\left( Q, (U / \{ u_{\sigma_{1}}, \ldots, u_{\sigma_{i - 1}} \}) / u_{\sigma_{i}}, 0 \right) \right)
\end{aligned}
\label{eq:pre_proof}
\end{equation}
% 记 $s_{i} = f\left( Q, U / \{ u_{\sigma_{1}}, \ldots, u_{\sigma_{i}} \}, 0 \right)$，构造如下 $g \in \mathcal{L}$：
Define $s_{i} = f\left( Q, U / \{ u_{\sigma_{1}}, \ldots, u_{\sigma_{i}} \}, 0 \right)$, and consider the following function $g \in \mathcal{R}$.
\begin{equation}
g( Q, U / \{ u_{1}, \ldots, u_{j} \}, s ) = 
\begin{cases}
s_{i}, 
  &j < \sigma_{i}, \\ 
  &s = s_{i} \\
s_{i},  
  &j = \sigma_{i}, \\ 
  &s = s_{i - 1} \\
s_{i - 1},  
  &j > \sigma_{i}, \\ 
  &s = s_{i - 1} \\
0, & \text{otherwise}
\end{cases}
\end{equation}
% 此时，有：
Consequently, we can derive the following:
\begin{equation}
\begin{aligned}
g^{m}(Q, U, 0) &= g^{m - 1}\left( Q, U, g^{m - 1}(Q, U, 0) \right)\\
&= g^{m - 1}(Q, U, s_{1})\\
&= \ldots\\
% &= g\left( Q, U, s_{m - 1} \right)\\
&= g\left( Q, 0, s_{m} \right)\\
&= f\left( Q, 0, s_{m} \right)\\
&= f(Q, U, 0)
\end{aligned}
\end{equation}
% 具体来讲，我们的方法用遍历一遍完整的表格来模拟Long CoT的一次状态转换，经过m次遍历达到Long CoT的最终状态s_m
Specifically, \ours simulates a state transition of Long CoT by traversing the entire table once.
After $m$ such traversals, \ours reaches the final state $s_m$ of Long CoT.
Therefore, Long CoT is a subset of \ours on the table reasoning task.



